Attribute-specific Control Units in StyleGAN for Fine-grained Image Manipulation

Image manipulation with StyleGAN has been an increasing concern in recent years.Recent works have achieved tremendous success in analyzing several semantic latent spaces to edit the attributes of the generated images.However, due to the limited semantic and spatial manipulation precision in these latent spaces, the existing endeavors are defeated in fine-grained StyleGAN image manipulation, i.e., local attribute translation.To address this issue, we discover attribute-specific control units, which consist of multiple channels of feature maps and modulation styles. Specifically, we collaboratively manipulate the modulation style channels and feature maps in control units rather than individual ones to obtain the semantic and spatial disentangled controls. Furthermore, we propose a simple yet effective method to detect the attribute-specific control units. We move the modulation style along a specific sparse direction vector and replace the filter-wise styles used to compute the feature maps to manipulate these control units. We evaluate our proposed method in various face attribute manipulation tasks. Extensive qualitative and quantitative results demonstrate that our proposed method performs favorably against the state-of-the-art methods. The manipulation results of real images further show the effectiveness of our method.

==> sections/temp_intro.tex <==

StyleGAN~\cite{karras2019style, karras2020analyzing}, as a state-of-the-art GAN, can synthesize diverse images with high quality.
%
The StyleGAN generator maps the random sampled noises to the intermediate latent codes and then further transforms them into hierarchical styles that modulate the hidden features.
%
By analyzing and identifying semantics in the latent representations of StyleGAN, we can reuse existing pre-trained StyleGAN to manipulate the synthesized images, which has a wide range of applications. 

Previous studies have explored hidden semantics learned by StyleGAN in numerous ways.
%
%This semantic knowledge are then used to guide to archive disentangled manipulation.
%
Previous works~\cite{goetschalckx2019ganalyze,jahanian2019steerability,harkonen2020ganspace,wang2021hijack} found that rich semantic information is encoded in the latent space of StyleGAN (e.g., $\mathcal{Z}$ or $\mathcal{W}$ space) and various semantic manipulations can be achieved by moving the latent code along the direction in the latent space.
%
For instance, InterfaceGAN~\cite{shen2020interfacegan} considers semantics are encoded in the linear subspace in the latent space of StyleGAN.
%
Therefore moving the latent code close to or away from the separating hyperplane in the latent space of the desired attribute can manipulate the attribute of generated images.








Recent studies~\cite{bau2019gandissect,shen2020interfacegan} have found that a well-trained StyleGAN spontaneously encodes numerous semantic information in the latent space and hidden features, despite the absence of explicit supervision during training.


%
Some papers~\cite{spingarn2020gan,shen2021closedform} examined the internal representation in the generator's weights and determined meaningful latent space trajectories directly from the pre-trained weights without any training or optimization.
%
Modifications to the latent code in the $\mathcal{Z}$ or $\mathcal{W}$ space lack explicit control over the modified region. Therefore, while the target attribute of the generated images is successfully manipulated using their methods, irrelevant regions and attributes in the image are usually also changed.
%

\begin{figure}[t]
\begin{center}
\includegraphics[width=1.0\linewidth]{./pics/fig1.pdf}
\end{center}
\caption{
Both critical modulation styles and feature maps need to be manipulated to add a full beard.
(a) The original StyleGAN generation process. (b) Manipulate a few channels of the $l^{th}$ layer's modulation styles $S^l$ by moving it along with a sparse direction $\Delta{S^l}$. (c) Manipulate a few feature channels and their corresponding modulation styles at the same time.
%
Gray feature maps indicate that they have been modified.
}\label{fig:fig1}
\end{figure}


% GAN Dissection~\cite{bau2019gandissect} identifies feature channels with a causal relationship with specific object concepts and manipulates the existence of a visual object in the generated image by directly modifying these feature maps.
% %
% However, for local attribute manipulation tasks, our goal is usually not to control the presence or absence of some semantic regions but to manipulate the attribute of these regions.
% %

% 应该更快的进入特征层面的叙述，现在前面的太长了。
A recent work StyleSpace~\cite{wu2020stylespace} further finds that the feature map's modulation styles at different scales are rich in semantic information and more disentangled than other intermediate latent representations.
%
Spatial disentangled manipulation can be achieved by modifying only a single feature channel's manipulation style.
%
We believe that this is because adjusting the modulation parameters of a single channel brings about a change in the following feature maps consistent with this channel of feature's spatial distribution.
%
GAN Dissection~\cite{bau2019gandissect} finds that the top activated spatial location in feature maps align with specific semantic regions across a variety of generated images.
%
So these single-channel controls bring consistent attribute manipulations on the diverse generated images.
%
However, we found that the results manipulated by these single-channel controls still suffer from insufficient change issues, especially when the feature maps corresponding to these single-channel controls are not complete.
%
More importantly, many semantic attributes are not just controlled by one style channel.

% 其实本质是一共有N层style，最后几层只控制纹理细节
% 那么一定存在一个第l+1层，只要把l+1层特征更改为我们期望的就可以实现编辑目标
% 计算得到l+1层特征需要第l层的style和第l层的特征，前l-1层的style信息已经完全包含在l层特征中。
% 其它前l层style都修改的方法本质上也是在修改第l层特征和l层style
Inspired by the above observations, we infer that the semantics of a specific region in the image is encoded both in a few channels of intermediate features and the modulation styles corresponding to them.
%
We can roughly divide each channel of the feature in a particular layer into multiple groups by the top activated spatial location.
%
Each channel group is specialized to synthesize a certain semantic region in the generated images.
%
We should modify only the features and modulation styles in its corresponding group to manipulate a specific semantic region without affecting other regions in synthesized images.

Like StyleSpace, editing only the modulation styles of just a few channels may bring about the desired attribute change. 
%
However, the spatial distribution of the differences brought about by manipulation depends on the spatial distribution of these feature maps.
%
It thus may still suffer from issues like spatial entanglement and insufficient change.
%
As shown in Fig.~\ref{fig:fig1}b, although we successfully added the goatee, the shape of the goatee is not complete enough, which aligns with the highly activated part of the feature maps.
%
We thus believe that in addition to modifying several style channels, the corresponding feature maps should also be modified to improve the manipulation effect.
After modifying the high activation part of the feature maps to align with the chin and mouth of the face, the same modulation styles moving direction produces a full goatee, as shown in Fig.~\ref{fig:fig1}c.

In this work, we first introduce a simple yet effective backpropagation-based strategy to determine the semantic regions with consistently high activation for each feature channel. 
%
Each feature channel in the same layer is then divided into multiple groups according to the highly activated semantic regions. 
%
We then find sparse semantic direction vectors by various methods 
% 比如只有两个正负样本？
that modify only the modulation styles in the group corresponding to the target semantic region.
%
The feature maps corresponding to the modified modulation parameters are also replaced to activate in the target semantic region to enhance the effectiveness and disentanglement of attribute manipulation.
%
As a result, our proposed method can bring a disentangled and effective manipulations along various local attributes.

Our main contributions could be summarized as follows:

\begin{itemize}
    \item We demonstrate that each channel of StyleGAN intermediate features and its modulation parameters are responsible for synthesizing different semantic regions in the synthesized image. We then propose a simple yet effective method to identify the regions responsible for each channel.
    
    \item We propose a move-replace strategy for attribute manipulation, which consists of replacing feature maps and the movement of modulation styles in critical units for a specific attribute of semantic region. It can achieve the disentangled and effective controls along various local attributes.
   
   \item We validate the effectiveness of our approach with the task of facial attribute editing. Extensive qualitative results show that our method can achieve spatial and semantic disentangled StyleGAN controls, while keeping the visual fidelity of generated images.
\end{itemize}
